From multiple unitarity cuts to the coproduct of Feynman integrals

We develop techniques for computing and analyzing multiple unitarity cuts of Feynman integrals, and reconstructing the integral from these cuts. We study the relations among unitarity cuts of a Feynman integral computed via diagrammatic cutting rules, the discontinuity across the corresponding branch cut, and the coproduct of the integral. For single unitarity cuts, these relations are familiar. Here we show that they can be generalized to sequences of unitarity cuts in different channels. Using concrete one- and two-loop scalar integral examples we demonstrate that it is possible to reconstruct a Feynman integral from either single or double unitarity cuts. Our results offer insight into the analytic structure of Feynman integrals as well as a new approach to computing them.

==> App_DiscSingleCuts.tex <==
\section{Explicit results for the discontinuity of single unitarity cuts on the $p_3^2$-channel}

We start by explaining how the analytical continuation of multiple polylogarithms is done, and then
give explicit results for the discontinuity of the single unitarity cuts on the $p_3^2$-channel given in Appendix~\ref{singleCutRes}
across the branch cut starting at $\zbar=0$.

\subsection{Analytical continuation of multiple polylogarithms}

The results we gave in the previous section were computed in a very specific region of the ($z$, $\zbar$) variables, where they are the complex conjugate of each other.
However, we now want to compute the discontinuities of the above cuts across the branch cut starting at $\zbar=0$, in the region where $\zbar<0$ and $0<z<1$.

To compute the discontinuity of a function across a given branch cut, we first analytically continue the function from the region where it was computed to one side of the cut, then to the other
side of the cut, and finally take the difference of the two analytical continuations. When doing this, we need to be sure we stay in the same sheet.

The analytical continuation of the function is completely determined by the $i\varepsilon$ prescription of the propagators. Indeed, a $\pm i\varepsilon$ in the propagator
leads to a $\pm i\varepsilon$ in the kinematic invariants on which the amplitude depends and thus, for example:
\begin{equation}
\ln(-p_i^2)=\ln\left(-(p_i^2\pm i\varepsilon)\right)=\ln\abs{p_i^2}\mp i \pi \theta\left(p_i^2\right)
\end{equation}
For an amplitude $\mathcal{A}$, where the propagators have a $+i\varepsilon$, the discontinuity across a branch cut associated with the $p_i^2$ invariant is given by:
\begin{equation}
\Disc_{p_i^2}\mathcal{A}(p_i^2)=\mathcal{A}(p_i^2+i\varepsilon)-\mathcal{A}(p_i^2-i\varepsilon)
\end{equation}

While the analytical continuation for logarithms is trivial, for more complicated multiple polylogarithms it becomes quite hard. However, using the
extended Hopf algebra of multiple polylogarithms \cite{Duhr:2012fh} it can be done in an algorithmic way. We now explain this procedure based on a specific examples.\\

We start with a weight 2 function, $G(1,0,\zbar)$, which we will continue to the region where $\zbar<0$, and $\zbar=\zbar+i\varepsilon$.
We begin by computing the symbol of this function:
\begin{equation*}
\mathcal{S}\left[G(1,0,\zbar)\right]=\zbar\otimes (1-\zbar)
\end{equation*}
The first thing we can notice is that given that $\zbar$ appears as the first entry in some of these terms, the function does have a branch point at $\zbar=0$.
Acting with $\Delta_{1,1}$ on the function:
\begin{align*}
\Delta_{1,1}\left[G(1,0,\zbar+i\varepsilon)\right]=&G(0,\zbar)\otimes G(1,\zbar)\\
=&G(0,-\zbar)\otimes G(1,\zbar)+i \pi\otimes G(1,\zbar)\\
=&G(0,-\zbar)\otimes G(-1,-\zbar)+i \pi\otimes G(1,\zbar)\\
=&\Delta_{11}\left[G(-1,0,-\zbar)+i \pi G(1,\zbar)\right]
\end{align*}
and thus:
\begin{equation*}
G(1,0,\zbar+i\varepsilon)=G(-1,0,-\zbar)+i \pi G(1,\zbar)+k\zeta_2
\end{equation*}
The value of $k$ can be determined numerically, and we find $k=0$. All the functions on the right-hand side are away from the $\zbar$ branch cut, by which we mean:
\begin{equation}
G(...,\zbar+i\varepsilon,...)-G(...,\zbar-i\varepsilon,...)=\mathcal{O}(\varepsilon)
\label{noDisc}
\end{equation}
Finally, in the same way:
\begin{equation*}
G(1,0,\zbar-i\varepsilon)=G(-1,0,-\zbar)-i \pi G(1,\zbar)
\end{equation*}
We can now compute the discontinuity of this function:
\begin{equation}
\Disc_{\zbar=0}=G(1,0,\zbar+i\varepsilon)-G(1,0,\zbar-i\varepsilon)=2\pi i G(1,\zbar)
\end{equation}
The analytical continuation and thus also the discontinuity of all weight 2 functions can be computed in this way.\\

We now go on to a more complicated example, a weight 3 function depending on both $z$ and $\zbar$.
We will compute the analytical continuation of $G(z,1,0,\zbar+i\varepsilon)$ from the region $\zbar=z^*$ to the region $\zbar<0$, $0<z<1$, with $\zbar=\zbar+i\varepsilon$.
We start by computing the symbol of this function:
\begin{align}
\mathcal{S}\left[G(z,1,0,\zbar)\right]=&
(z-\zbar)\otimes z\otimes (1-z)-\zbar\otimes z\otimes (1-z)-\zbar\otimes (1-\zbar)\otimes (1-z)\nonumber\\
&+\zbar\otimes (1-\zbar)\otimes (z-\zbar)+\zbar\otimes (z-\zbar)\otimes (1-z)-(z\otimes z\otimes (1-z))
\end{align}
We notice there is indeed a branch point at $\zbar=0$.
Because we know that in this region $z$ is far from any branch cut, we `integrate' the symbol to get functions of $z$ whenever possible:
\begin{align}
\mathcal{S}\left[G(z,1,0,\zbar)\right]=\mathcal{S}&\big[G(1,z) G(0,0,\zbar)-G(1,z) G(1,0,\zbar)+G(1,0,\zbar) G(\zbar,z)
+G(0,\zbar) G(1,\zbar,z)\big.\nonumber\\
&\big.+G(1,0,\zbar,z)-G(1,0,0,z)+G(0,1,0,\zbar)\big]
\end{align}
Under the symbol sign, we now do all the analytical continuations we know how to do. In particular, all weight one functions can be analytically continued trivially:
\begin{align*}
G(0,\zbar+i\varepsilon)&=\ln\left(\zbar+i\varepsilon\right)=G(0,-\zbar)+i \pi\\
G(1,z)&=\ln\left(1-z\right)=G(1,z)\\
G(\zbar+i\varepsilon,z)&=\ln\left(1-\frac{z}{\zbar+i \varepsilon}\right)=G(\zbar,z)
\end{align*}
The continuation of all weight 2 functions will have been computed previously. The results we need are:
\begin{align*}
G(0,0,\zbar\pm i\varepsilon)&=\pm i \pi  G(0,-\zbar)+G(0,0,-\zbar)-\frac{\pi ^2}{2}\\
G(1,0,\zbar\pm i\varepsilon)&=G(-1,0,-\zbar)\pm i \pi G(1,\zbar)\\
G(1,\zbar\pm i\varepsilon,z)&=G(1,\zbar,z)
\end{align*}
Finally, the continuation of the weight 3 function $G(0,1,0,\zbar)$ can be done exactly as the weight 2 example we gave above so we only give the result:
\begin{equation*}
G(0,1,0,\zbar\pm i\varepsilon)=G(0,-1,0,-\zbar)\pm i \pi  G(0,1,\zbar)
\end{equation*}
We thus have:
\begin{align*}
\mathcal{S}\left[G(z,1,0,\zbar+ i\varepsilon)\right]=\mathcal{S}&\Big[
-G(1,z) G(-1,0,-\zbar)+G(-1,0,-\zbar) G(\zbar,z)+G(1,z) G(0,0,-\zbar)\Big.\\
&+G(0,-\zbar) G(1,\zbar,z)+G(1,0,\zbar,z)-G(1,0,0,z)+G(0,-1,0,-\zbar)\\
&+i \pi  G(1,z) G(0,-\zbar)-i \pi  G(1,z) G(1,\zbar)+i \pi  G(1,\zbar) G(\zbar,z)+i \pi  G(1,\zbar,z)\\
\Big.&+i \pi  G(0,1,\zbar)
-\frac{1}{2} \pi ^2 G(1,z)\Big]\\
\equiv\mathcal{S}&\Big[G_{\mathcal{S}}(z,\zbar+ i\varepsilon)\Big]
\end{align*}
We now act with $\Delta_{1,1,1}$ on the difference between the left-hand side and the right-hand side  to look for missing terms of the form $i \pi G(a,b,c)$:
\begin{equation*}
\Delta_{1,1,1}\Big[G(z,1,0,\zbar+ i\varepsilon)-G_{\mathcal{S}}(z,\zbar+ i\varepsilon)\Big]=-i \pi \otimes G(0,z)\otimes G(1,z)
\end{equation*}
and define:
\begin{equation*}
G_{\Delta_{1,1,1}}(z,\zbar+ i\varepsilon)=G_{\mathcal{S}}(z,\zbar+ i\varepsilon)+i \pi G(1,0,z)
\end{equation*}
so that:
\begin{equation*}
\Delta_{1,1,1}\Big[G(z,1,0,\zbar+ i\varepsilon)-G_{\Delta_{1,1,1}}(z,\zbar+ i\varepsilon)\Big]=0
\end{equation*}
Finally, we look for missing terms of the form $\pi^2G(a,b)$:
\begin{equation*}
\Delta_{2,1}\Big[G(z,1,0,\zbar+ i\varepsilon)-G_{\Delta_{1,1,1}}(z,\zbar+ i\varepsilon)\Big]=\frac{1}{3} \pi ^2\otimes G(1,z)
\end{equation*}
and again define:
\begin{equation*}
G_{\Delta_{2,1}}(z,\zbar+ i\varepsilon)=G_{\Delta_{1,1,1}}(z,\zbar+ i\varepsilon)+\frac{1}{3} \pi ^2 G(1,z)
\end{equation*}
At this stage, we can only be missing constant terms, which at weight 3 are either $i \pi^3$ and $\zeta_3$:
\begin{equation*}
G(z,1,0,\zbar+ i\varepsilon)-G_{\Delta_{2,1}}(z,\zbar+ i\varepsilon)=k\zeta_3+n\, i\pi^3
\end{equation*}
Numerically, we find $k=n=0$. We thus finally have:
\begin{align*}
G(z,1,0,\zbar+ i\varepsilon)=&
-G(1,z) G(-1,0,-\zbar)+G(-1,0,-\zbar) G(\zbar,z)+G(1,z) G(0,0,-\zbar)\\
&+G(0,-\zbar) G(1,\zbar,z)+G(1,0,\zbar,z)-G(1,0,0,z)+G(0,-1,0,-\zbar)\\
&+i \pi  G(1,z) G(0,-\zbar)-i \pi  G(1,z) G(1,\zbar)+i \pi  G(1,\zbar) G(\zbar,z)+i \pi  G(1,\zbar,z)\\
&-i \pi  G(1,0,z)+i \pi  G(0,1,\zbar)-\frac{1}{6} \pi ^2 G(1,z)
\end{align*}
Again, all the functions on the right-hand side satisfy \refE{noDisc} so are away from the branch cut.

The same calculation can be made with $\zbar=\zbar- i\varepsilon$. We get:
\begin{align*}
G(z,1,0,\zbar- i\varepsilon)=&
-G(1,z) G(-1,0,-\zbar)+G(-1,0,-\zbar) G(\zbar,z)+G(1,z) G(0,0,-\zbar)\\
&+G(0,-\zbar) G(1,\zbar,z)+G(1,0,\zbar,z)-G(1,0,0,z)+G(0,-1,0,-\zbar)\\
&-i \pi  G(1,z) G(0,-\zbar)+i \pi  G(1,z) G(1,\zbar)-i \pi  G(1,\zbar) G(\zbar,z)-i \pi  G(1,\zbar,z)\\
&+i \pi  G(1,0,z)-i \pi  G(0,1,\zbar)-\frac{1}{6} \pi ^2 G(1,z)
\end{align*}
and thus the discontinuity of $G(z,1,0,\zbar)$ is:
\begin{align}
\Disc_{\zbar=0}G(z,1,0,\zbar)=&G(z,1,0,\zbar+ i\varepsilon)-G(z,1,0,\zbar- i\varepsilon)\nonumber\\
=&2 i \pi  G(1,z) G(0,-\zbar)-2 i \pi  G(1,z) G(1,\zbar)+2 i \pi  G(1,\zbar) G(\zbar,z)\nonumber\\
&+2 i \pi  G(1,\zbar,z)-2 i \pi  G(1,0,z)+2 i \pi  G(0,1,\zbar)
\end{align}\\

All the analytical continuations we need to compute can be done in this way. Moreover, this method can be generalised to higher weight functions
in a straightforward way.

\subsection{Discontinuity across the $p_1^2$ branch cut of the single unitarity cuts on the $p_3^2$-channel}

We give the results for the discontinuity of the single unitarity cuts on the $p_3^2$-channel, in the region $\zbar<0$, $0<z<1$.

\subsubsection{Discontinuity across the $p_1^2$ branch cut of cut (45)}

\begin{align}
\Disc_{\zbar=0}f^{(45)}_{-2}=-4 i\pi
\end{align}

\begin{align}
\Disc_{\zbar=0}f^{(45)}_{-1}=-8 i \pi  G(\zbar,z)+4 i \pi  G(0,z)+8 i \pi  G(1,z)-4 i \pi  G(0,-\zbar)+8 i \pi  G(1,\zbar)+4 \pi ^2
\end{align}

\begin{align}
\Disc_{\zbar=0}f^{(45)}_{0}=&4 i \pi  G(0,z) G(0,-\zbar)+8 i \pi  G(1,z) G(0,-\zbar)-8 i \pi  G(0,-\zbar) G(\zbar,z)-8 i \pi  G(0,z) G(1,\zbar)\nonumber\\
&-16 i \pi  G(1,z) G(1,\zbar)+16 i \pi  G(1,\zbar) G(\zbar,z)+8 i \pi  G(0,\zbar,z)+16 i \pi  G(1,\zbar,z)\nonumber\\
&+8 i \pi  G(\zbar,0,z)+16 i \pi  G(\zbar,1,z)-16 i \pi  G(\zbar,\zbar,z)-4 i \pi  G(0,0,z)-8 i \pi  G(0,1,z)\nonumber\\
&-8 i \pi  G(1,0,z)-16 i \pi  G(1,1,z)+8 i \pi  G(1,\zbar) G(0,-\zbar)-4 i \pi  G(0,0,-\zbar)-16 i \pi  G(1,1,\zbar)\nonumber\\
&+8 \pi ^2 G(\zbar,z)-4 \pi ^2 G(0,z)-8 \pi ^2 G(1,z)+4 \pi ^2 G(0,-\zbar)-8 \pi ^2 G(1,\zbar)
+\frac{8 i \pi ^3}{3}
\end{align}

\subsubsection{Discontinuity across the $p_1^2$ branch cut of cut (12)}

\begin{align}
\Disc_{\zbar=0}f^{(12)}_{-2}=-4 i\pi
\end{align}

\begin{align}
\Disc_{\zbar=0}f^{(12)}_{-1}=-8 i \pi  G(\zbar,z)+4 i \pi  G(0,z)+8 i \pi  G(1,z)-4 i \pi  G(0,-\zbar)+8 i \pi  G(1,\zbar)-4 \pi ^2
\end{align}

\begin{align}
\Disc_{\zbar=0}f^{(12)}_{0}=&12 i \pi  G(0,z) G(0,-\zbar)+8 i \pi  G(1,z) G(0,-\zbar)-8 i \pi  G(0,-\zbar) G(\zbar,z)-8 i \pi  G(0,z) G(1,\zbar)\nonumber\\
&-16 i \pi  G(1,z) G(1,\zbar)+16 i \pi  G(1,\zbar) G(\zbar,z)+8 i \pi  G(0,\zbar,z)+16 i \pi  G(1,\zbar,z)\nonumber\\
&+8 i \pi  G(\zbar,0,z)+16 i \pi  G(\zbar,1,z)-16 i \pi  G(\zbar,\zbar,z)-12 i \pi  G(0,0,z)-8 i \pi  G(0,1,z)\nonumber\\
&-8 i \pi  G(1,0,z)-16 i \pi  G(1,1,z)+8 i \pi  G(-1,0,-\zbar)-4 i \pi  G(0,0,-\zbar)+8 i \pi  G(0,1,\zbar)\nonumber\\
&-16 i \pi  G(1,1,\zbar)-8 \pi ^2 G(\zbar,z)+4 \pi ^2 G(0,z)+8 \pi ^2 G(1,z)-4 \pi ^2 G(0,-\zbar)\nonumber\\
&+8 \pi ^2 G(1,\zbar)+\frac{8 i \pi ^3}{3}
\end{align}

\subsubsection{Discontinuity across the $p_1^2$ branch cut of cut (234)}

\begin{align}
\Disc_{\zbar=0}f^{(234)}_{-2}=4 i\pi
\end{align}

\begin{align}
\Disc_{\zbar=0}f^{(234)}_{-1}=8 i \pi  G(\zbar,z)-4 i \pi  G(0,z)-8 i\pi  G(1,z)+8 i \pi  G(0,-\zbar)-8 i \pi  G(1,\zbar)
\end{align}

\begin{align}
\Disc_{\zbar=0}f^{(234)}_{0}=&-8 i \pi  G(0,z) G(0,-\zbar)-16 i \pi  G(1,z)G(0,-\zbar)+16 i \pi  G(0,-\zbar) G(\zbar,z)\nonumber\\
&+8 i \pi  G(0,z) G(1,\zbar)+16 i \pi  G(1,z) G(1,\zbar)-16 i \pi  G(1,\zbar) G(\zbar,z)-4 i \pi  G(0,\zbar,z)\nonumber\\
&-16 i \pi  G(1,\zbar,z)-8 i \pi  G(\zbar,0,z)-16 i \pi  G(\zbar,1,z)+16 i \pi  G(\zbar,\zbar,z)+4 i \pi  G(0,0,z)\nonumber\\
&+8 i \pi  G(0,1,z)+8 i \pi  G(1,0,z)+16 i \pi  G(1,1,z)-16 i \pi  G(1,\zbar) G(0,-\zbar)+4 i \pi  G(0,0,-\zbar)\nonumber\\
&+12 i \pi  G(0,1,\zbar)+16 i \pi  G(1,1,\zbar)
-4 i \pi ^3
\end{align}

\subsubsection{Discontinuity across the $p_1^2$ branch cut of cut (135)}

\begin{align}
\Disc_{\zbar=0}f^{(135)}_{-2}=4 i\pi
\end{align}

\begin{align}
\Disc_{\zbar=0}f^{(135)}_{-1}=8 i \pi  G(\zbar,z)-4 i \pi  G(0,z)-8 i \pi  G(1,z)-8 i \pi  G(1,\zbar)
\end{align}

\begin{align}
\Disc_{\zbar=0}f^{(135)}_{0}=&-4 i \pi  G(0,z) G(0,-\zbar)+8 i \pi  G(0,z) G(1,\zbar)+16 i \pi  G(1,z) G(1,\zbar)-16 i \pi  G(1,\zbar) G(\zbar,z)\nonumber\\
&-12 i \pi  G(0,\zbar,z)-16 i \pi  G(1,\zbar,z)-8 i \pi  G(\zbar,0,z)-16 i \pi  G(\zbar,1,z)+16 i \pi  G(\zbar,\zbar,z)\nonumber\\
&+8 i \pi  G(0,0,z)+8 i \pi  G(0,1,z)+8 i \pi  G(1,0,z)+16 i \pi  G(1,1,z)+4 i \pi  G(0,0,-\zbar)\nonumber\\
&-12 i \pi  G(0,1,\zbar)+16 i \pi  G(1,1,\zbar)
-\frac{4 i \pi ^3}{3}
\end{align}


